Complex-Valued Neural Networks for Ultra-Reliable Massive MIMO

In the evolving landscape of 5G and 6G networks, the demands extend beyond high data rates, ultra-low latency, and extensive coverage, increasingly emphasizing the need for reliability. This paper proposes an ultra-reliable multiple-input multiple-output (MIMO) scheme utilizing quasi-orthogonal space-time block coding (QOSTBC) combined with singular value decomposition (SVD) for channel state information (CSI) correction, significantly improving performance over QOSTBC and traditional orthogonal STBC (OSTBC) when analyzing spectral efficiency. Although QOSTBC enhances spectral efficiency, it also increases computational complexity at the maximum likelihood (ML) decoder. To address this, a neural network-based decoding scheme using phase-transmittance radial basis function (PT-RBF) architecture is also introduced to manage QOSTBC's complexity. Simulation results demonstrate improved system robustness and performance, making this approach a potential candidate for ultra-reliable communication in next-generation networks.

==> temp.tex <==
\subsection{Space-Time Block Coding and OFDM}
\label{sub:STBC}

A generalized coding scheme referred to as space-time block codes (STBCs)~\cite{Jankiraman2004,Tarokh1999,Li2021}, based on the theory of orthogonal matrix designs, can achieve the full-transmit diversity of $N_{tx} N_{rx}$ employing the maximum likelihood~(ML) decoding algorithm at the receiver~\cite{Jankiraman2004}. The idea is to transmit $N_{tx}$ orthogonal streams, which implies that the receiver antennas receive $N_{tx}$ orthogonal streams. This special class of space-time block codes is the so-called orthogonal STBC (OSTBC) \cite{soares2021,Tarokh1999,Hu2020}. Besides diversity gain, the OSTBC leads to a secondary linear coding gain $G_c = 10\log\left(R\right)$ at the receiver due to the coherent detection of multiple signal copies over time, and an array gain $G_a = 10\log\left(N_{rx}\right)$ due to the coherent combination of multiple received signals over the receiving antennas~\cite{soares2021}.


One of the disadvantages of OSTBC is the code rate. Let $N_{tp}$ represent the number of time samples to convey one block of coded symbols and $N_s$ represent the number of symbols transmitted per block. The space-time block code rate is defined as the ratio between the number of symbols that the encoder receives at its input and the number of space-time coded symbols transmitted from each antenna, given by $R = N_s/N_{tp}$. For example, an OSTBC coding matrix for $N_{tx}=4$ implies a code rate $R=1/2$, reducing spectral efficiency.


In order to increase the spectral efficiency in orthogonal codes, Jafarkhani~\cite{Jafarkhani898239} proposed quasi-orthogonal STBC (QOSTBC) of rate one, relaxing the requirement of orthogonality. However, when compared with orthogonal codes, the diversity gain is reduced by a factor of two. In contrast to orthogonally designed codes that process one symbol at a time on the decoder, quasi-orthogonal codes process pairs of transmitted symbols, which exponentially increases the computational complexity of decoding~\cite{soares2021}. Jafarkhani~\cite{Jafarkhani898239} proposed a coding matrix of rate one for $N_{tx}=4$, given by

\begin{equation}
    \label{eq:QOSTBC44}
    \mathbf{QOSTBC_{4,4}}=\begin{bmatrix}
   s[1] & s[2] & s[3] & s[4]\\ 
   -s[2]^* & s[1]^* & -s[4]^* & s[3]^*\\
   -s[3]^* & -s[4]^* & s[1]^* & s[2]^*\\
   s[4] & -s[3] & -s[2] & s[1]\\
    \end{bmatrix}.
\end{equation}

In the literature, related approaches with a maximum of $N_{tx}=6$ antennas were proposed for quasi-orthogonal codes~\cite{TBH876470,Weifeng1188366,SindhuHameed7383923}. In~\cite{Weifeng1188366}, the authors developed an architecture similar to~\cite{Jafarkhani898239}; however, it presents full diversity at the cost of more processing and is limited to $N_{tx}=4$ antennas. In the same way, by increasing the decoding processing, Sindhu and Hameed~\cite{SindhuHameed7383923} proposed two quasi-orthogonal schemes with $N_{tx}=5$ and $6$ antennas~\cite{soares2021}.

\subsection{Quasi-Orthogonal Coding Scheme}

In the present paper, we use the generalized recursive method proposed in~\cite{soares2021} for generating QOSTBC coding schemes:
\begin{equation}
    \mathbf{S}_{N_s}^{N_{tx}} = 
    \begin{bmatrix}
    \mathbf{S}_{N_s-N_{tx}/2}^{N_{tx}/2} & \mathbf{S}_{N_s}^{N_{tx}/2}\\ 
    -[{\mathbf{S}_{N_s}^{N_{tx}/2}}]^* & [{\mathbf{S}_{N_s-N_{tx}/2}^{N_{tx}/2}}]^*
    \end{bmatrix},
    \label{eq:propCode}
\end{equation}
in which $N_{tx} = 2^n, \: \forall \: n \in \mathbb{N}^+$, is the number of transmitting antennas and $N_s$ is the number of encoded symbols. In this encoding approach, $N_s\triangleq N_{tx}$ and the code rate is $R=N_{tx}/N_s = 1$~\cite{soares2021}. The recurrence is employed until ${\mathbf{S}_{n}^{1}}=s[n] ,\, \forall n \in [1,\,2,\cdots,N_s]$ in~\eqref{eq:propCode}.

With four transmitting antennas,~\eqref{eq:propCode} results in:

\begin{equation}
    \label{eq:S4}
    \mathbf{S}_{4}^{4} =
    \begin{bmatrix}
        s[1] & s[2] & s[3] & s[4] \\ 
        -s[2]^* & s[1]^* & -s[4]^* & s[3]^* \\ 
        -s[3]^* & -s[4]^* & s[1]^* & s[2]^* \\ 
        s[4] & -s[3] & -s[2] & s[1]
    \end{bmatrix}.
\end{equation}

Note that \eqref{eq:S4} is equal to the coding scheme proposed by~\cite{Jafarkhani898239} with four antennas, as in~\eqref{eq:QOSTBC44}. However, in contrast to the work of~\cite{Jafarkhani898239}, this scheme can generate coding matrices for any $N_{tx} = 2^n, \: \forall \: n \in \mathbb{N}^+$, and $N_s\triangleq N_{tx}$~\cite{soares2021}. For the case of $n=1$, \eqref{eq:propCode} is equal to the Alamouti coding, the full-rate full-diversity complex-valued space-time block code proposed in~\cite{Alamouti730453}.

